Data-Association-Free Landmark-based SLAM

We study landmark-based SLAM with unknown data association: our robot navigates in a completely unknown environment and has to simultaneously reason over its own trajectory, the positions of an unknown number of landmarks in the environment, and potential data associations between measurements and landmarks. This setup is interesting since: (i) it arises when recovering from data association failures or from SLAM with information-poor sensors, (ii) it sheds light on fundamental limits (and hardness) of landmark-based SLAM problems irrespective of the front-end data association method, and (iii) it generalizes existing approaches where data association is assumed to be known or partially known. We approach the problem by splitting it into an inner problem of estimating the trajectory, landmark positions and data associations and an outer problem of estimating the number of landmarks. Our approach creates useful and novel connections with existing techniques from discrete-continuous optimization (e.g., k-means clustering), which has the potential to trigger novel research. We demonstrate the proposed approaches in extensive simulations and on real datasets and show that the proposed techniques outperform typical data association baselines and are even competitive against an "oracle" baseline which has access to the number of landmarks and an initial guess for each landmark.

==> includes/table-real-old.tex <==
%!TEX root = ../main.tex

\begin{table}[tb]
    \small
    \centering
    \noindent
    \caption{
        ATE (first two rows) and run-time (sec) (last two rows) results on the two real datasets. Estimates of the number of landmarks are given in parentheses (relative to the ground-truth). 
    }
    \begin{tabular}{c | c c c c c}
        \hline
        Dataset & Odom & ML & Alt & GNC & \nameKmeans  \\
        \hline
        Indoor & 0.415 (+24)  & 0.833 & 0.076 & 0.157 & \textbf{0.046} (+1) \\
        Corridor & 6.67 (+233) & 7.13 & 4.18 & 5.817 & \textbf{1.068} (-233) \\
        \hline
        Indoor & n/a & 7.49 & 1.66 & 2.94 & 16.73 \\
        Corridor & n/a & 77.05 & 24.83 & 21.93 & 69.2 \\
        \hline
    \end{tabular}
    \label{tab:realresults}
\end{table}

==> sections/experimentsOld.tex <==
%!TEX root = ../root.tex

\section{Experiments}
\label{sec:experiments}

\subsection{Baselines}

Our proposed algorithms are compared with (1) a simpler alternation scheme that has access to the ground-truth number of landmarks and an initial guess for each landmark, and (2) a more traditional incremental formulation of SLAM, where odometry is propagated sequentially and data association is made on the arriving measurements with the maximum likelihood estimator \cite{bar1990tracking}. 

The alternation baseline is quite simple. In the first step, it enumerates the landmark variables $\vy_j$ and finds the one that minimizes $\| \MR_{i_k}\tran \vy_{j}  \!-\! \vt_{i_k} \!-\! \vzbar_k \|^2$ to be the landmark that associates to measurement $\vzbar_k$ given the current estimates of $\vxx$ and $\vy$. After making associations for all the measurements, it solves the SLAM problem with the estimated associations. This process repeats until convergence. In contrast to Algorithm~\ref{algo:nameKmeans}, this baseline alternation solves only the data associations in the first step but not together with $\vy$. Thus, it requires an initial guess for each landmark to start with, inevitably also knowing the ground-truth number of landmarks.

% Unlike the JCBB method \cite{neira2001data}, the maximum likelihood approach is fast enough to test on real-world sized datasets. In our implementation of the maximum likelihood approach,  the data association process follows two stages. 

The incremental maximum likelihood approach follows two stages. The first stage is to perform a crude selection of landmarks by thresholding the Euclidean distance between the estimated landmark position for existing landmark variables $\vy_j$ and the transformed measurement position in the world frame for some range threshold $r_{\mathrm{thresh}}$, given by
\begin{equation}
\norm{\MR_{i_k}\tran\vy_j - \vt_{i_k} - \vzbar_k}_2 < r_{\mathrm{thresh}}. 
\end{equation}
This step forms an admissible set $\calA$ similar to the one in the GNC approach (Section~\ref{sec:solver-gnc}) to reduce computation load. Then, each of the landmarks that are in the admissible set is tested for \emph{individual compatibility} with a $\chi^2$-test dependent on the \emph{Mahalanobis distance} $\varepsilon_{kj}$ between the landmark $\vy_{j}$ and the measurement $\vz_{k}$, given by
\begin{equation}
    \varepsilon_{kj} = \left(\vzbar_k - h(\vxx_{i_k}, \vy_{j})\right)\tran\boldsymbol{S}^{-1}_{kj}\left(\vzbar_k - h(\vxx_{i_k}, \vy_{j})\right),
\end{equation}
where $h(\vxx_{i_k}, \vy_j)$ is the measurement model given in \eqref{eq:formulationLmkCount}, $\boldsymbol{S}_{kj}=\boldsymbol{H}_{kj}\boldsymbol{P}_{kj}\boldsymbol{H}_{kj}\tran + \boldsymbol{Q}_k$ is the covariance of the measurement likelihood, $\boldsymbol{H}_{kj}$ is the joint Jacobian of the measurement model with respect to the state $\vxx_{i_k}$ and the landmark $\vy_j$, $\boldsymbol{P}_{kj}$ is the joint marginal covariance for the state $\vxx_{i_k}$ and landmark $\vy_j$ and $\boldsymbol{Q}_k$ is the measurement noise covariance. The $\chi^2$-test is formulated as whether the the computed Mahalanobis distance $\varepsilon_{kj}$ satisfies
\begin{equation}
    \varepsilon_{kj} < \varepsilon_{\mathrm{thresh}}
\end{equation}
where $\varepsilon_{\mathrm{thresh}} = \texttt{chi2inv}(\alpha, \mathrm{dim}(\vz))$ for some probability threshold $\alpha$.

The second stage of the algorithm ensures the \emph{mutual exclusion principle} of data association. The first pass ensures that all measurements are associated with exactly one landmark, but may cause a landmark to have multiple measurement candidates. In the second stage, each landmark is associated with the measurement with the \emph{lowest negative loglikelihood score} $l_{kj}$, given by
\begin{equation}
    l_{kj} = \log(\det\left(\boldsymbol{S}_{kj}\right)) + \varepsilon_{kj}
\end{equation}
where common constant terms and factors are removed as they do not affect the solution to the optimization problem. The remaining measurements that are not associated to a landmark are initialized as new landmarks using the measurement in the world frame as the initial estimate.


\subsection{Datasets}

We evaluate our K-SLAM algorithm (Algorithm~\ref{algo:nameKmeans}) and GNC algorithm (Section~\ref{sec:solver-gnc}) along with the baselines on two fully synthetic "grid" datasets (2D and 3D), two semi-synthetic datasets where the trajectories are real, but the landmarks are synthetic, and two real datasets \cite{}. Fig.~\ref{fig:mapviz} shows example visualization of the six datasets.

For the two synthetic datasets, we first generate a grid-like ground-truth trajectory and uniformly sample landmark positions in a slightly enlarged space where the trajectory occupies. Gaussian noise is injected to the ground-truth trajectory to create odometry measurements and to the landmark measurements following eq.~\eqref{eq:ldmkmeasurement}. Each landmark is observed by a fixed number of poses that are closest in their ground-truth positions to the landmark. The initial guess for the poses is the odometry. The initial guess for a landmark (only used by the baseline alternation) is obtained by composing the initial guess of the closest pose and the measurement from that pose. Finally, we run Gauss-Newton optimization given the odometry and landmark measurements (with known data associations) to obtain the pseudo-ground-truth trajectory for our testing purpose. This pseudo-ground-truth represents the best any method could do without data association information.

For the two semi-synthetic datasets, we first use Gauss-Newton to optimize the original pose graph with loop closures. Landmarks are uniformly sampled in the space and landmark measurements are created with the optimized trajectory in the same manner as for the synthetic datasets. Loop closures are then discarded and only odometry is retained so that the methods rely on landmarks to close the loops. Initial guess is obtained in the same fashion as before. Gauss-Newton is again employed to obtain the pseudo-ground-truth given the odometry and landmark measurements.

In our synthetic and semi-synthetic experiments, we sweep through different parameter values that define the map (\eg odometry noise level, number of landmarks, and landmark measurement noise level). Five random simulations are performed for each set of parameters. The default map parameter values can be found in Tab.~\ref{tab:simparams}.

\begin{table}[t]
    \smaller
    \centering
    \noindent
    \caption{
        Dataset default parameters. Values in bold are varied in our experiments. n/a stands for a dense matrix not representable by a single value.
    }
    \begin{tabular}{c | c c c}
        % \hline
        % Dataset & 2D Grid & 3D Grid & Intel & Parking Garage & Indoor & Corridor  \\
        % \hline
        % \# of poses & 20 $\times$ 25 & 6 $\times$ 6 $\times$ 6 & 942 & 1661 & 571 & 1744 \\
        % \# of landmarks & \textbf{100} & \textbf{64} & \textbf{141} & \textbf{166} & 14 & 248 \\
        % \# of lm. measurements & $\times$ 12 & $\times$ 12 & $\times$ 15 & $\times$ 20 & 233 & 983 \\
        % odometry translation std. & \textbf{0.05} & \textbf{0.05} & 0.045 & 1 & 0.1 & (0.15, 0.05, 0.1) \\
        % odometry rotation std. & \textbf{0.005} & \textbf{0.01} & 0.014 & n/a & 0.1 & (0.003, 0.006, 0.006) \\
        % lm. measurement std. & \textbf{0.1} & \textbf{0.1} & \textbf{0.1} & \textbf{0.1} & 0.1 & 0.1 \\
        % \hline
        \hline
        Dataset & 2D Grid & 3D Grid & Intel \\
        \hline
        \# of poses & 20 $\times$ 25 & 6 $\times$ 6 $\times$ 6 & 942 \\
        \# of landmarks & \textbf{100} & \textbf{64} & \textbf{141} \\
        \# of lm. measurements & $\times$ 12 & $\times$ 12 & $\times$ 15 \\
        odometry translation std. & \textbf{0.05} & \textbf{0.05} & 0.045 \\
        odometry rotation std. & \textbf{0.005} & \textbf{0.01} & 0.014 \\
        lm. measurement std. & \textbf{0.1} & \textbf{0.1} & \textbf{0.1} \\
        \hline
        Dataset & Garage & Indoor & Corridor \\
        \# of poses & 1661 & 571 & 1744 \\
        \# of landmarks & \textbf{166} & 14 & 248 \\
        \# of lm. measurements  & $\times$ 20 & 233 & 983 \\
        odometry translation std. & 1 & 0.1 & (0.15, 0.05, 0.1) \\
        odometry rotation std. & n/a & 0.1 & (0.003, 0.006, 0.006) \\
        lm. measurement std. & \textbf{0.1} & 0.1 & 0.1 \\
        \hline
    \end{tabular}
    \label{tab:simparams}
\end{table}

The real dataset \cite{} was collected for a previous research effort to study the ambiguous data association problem with semantic information. This dataset features a forward moving robot that is observing AprilTags \cite{} along the trajectory. In this dataset, the only way to reduce the odometry drift is closing large loops which requires some form of data association information (\eg semantic information as in \cite{}). The lack of any data association information as in our case makes it particularly challenging. We also evaluate on a public dataset where the robot frequently re-observes a small set of landmarks in the environment, which is a different scenario than \cite{}. 

\begin{figure}[htb!]
    \centering
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/maps/vizmap_2dsyn.png}
        \caption{Grid (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/maps/vizmap_3dsyn.png}
        \caption{Grid (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/maps/vizmap_intelos.png}
        \caption{Intel (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/maps/vizmap_garage.png}
        \caption{Parking Garage (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/maps/vizmap_matlab.png}
        \caption{Indoor (3D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/maps/vizmap_kevin.png}
        \caption{Corridor (3D)}
    \end{subfigure}%
    \caption{Visualization of the datasets. The black trajectories and markers are the initial guess. The blue trajectories and markers are the pseudo-ground-truth obtained by Gauss-Newton.}
    \label{fig:mapviz}
\end{figure}


\subsection{Results: Accuracy}
The K-SLAM algorithm, GNC, and the baseline alternation all use the Levenberg-Marquardt optimizer. The Maximum Likelihood approach uses ISAM2 \cite{ISAM2} with the Dogleg optimizer \cite{Dogleg_Powell1970} in the back-end. We present the results of our simulations on the synthetic and semi-synthetic datasets in Fig.~\ref{fig:gridresults} and Fig.~\ref{fig:semisynresults}. Tab.~\ref{tab:realresults} reports the results on the two real datasets. We visualize the resulting trajectories for K-SLAM in Fig.~\ref{fig:realkslam}.

Our K-SLAM algorithm outperforms the others in the majority of the experiments. In many cases, it even surpasses the baseline alternation which knows the actual number of landmarks and is given an initial guess for the landmarks. One interesting trend as seen in Fig.~\ref{fig:gridresults} is that K-SLAM tends to underestimate the number of landmarks as the landmark measurement noise goes up. This is expected -- as the landmark measurement noise increases, the tolerance of wrong data associations raises since the landmark measurements are down-weighted compared to the odometry term $f_{\text{odom}} (\vxx)$. The $\beta K$ term in eq. \eqref{eq:formulationLmkCount} then drives the number of landmarks ($K$) down, as it is facing reduced penalties for wrong data associations. For the same reason, increasing odometry noise has the opposite effect of causing overestimation.

We take advantage of this observation to tackle the most challenging dataset, the Corridor, where all the other algorithms fail to nicely close the loop (Tab.~\ref{tab:realresults}). In our experiment, a very high landmark measurement noise model is artificially set in K-SLAM. This noise model has two effects, (1) encouraging underestimation of the number of landmarks and aggressive data associations, and (2) suppressing the negative effects of wrong data associations. It turns out that on a dataset such as the Corridor where the success of reducing odometry drift relies critically on closing large loops, the synergy of these two effects causes the algorithm to close those large loops without paying a price for making incorrect data associations in small loops along the trajectory.

The maximum likelihood baseline performs well on the fully synthetic datasets, but not on the semi-synthetic or real datasets. We attribute this behavior to its reliance on covariance information, which ultimately comes from the prescribed noise models, to make data associations. For the fully synthetic data, the noise model provided to the algorithm matches exactly the actual noise characteristics. However, on semi-synthetic and real datasets, this perfect match is unlikely. The maximum likelihood suffers from this mismatch. Additionally, we observe its strong tendency to overestimate the number of landmarks.

GNC performs moderately in our experiments, with stable performance. We consider the strength of it lies in the speed-accuracy trade-off (Section~\ref{sec:runtime}).

\begin{figure}
    \centering
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0133_odom_noise_lv_rerun_refGN.png}
        % \caption{Grid (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0133_odom_noise_lv_rerun_nLm.png}
        % \caption{Grid (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0257_ldmk_t_std_rerun_refGN.png}
        % \caption{Intel (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0257_ldmk_t_std_rerun_nLm.png}
        % \caption{Parking Garage (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0217_ldmk_percent_rerun_refGN.png}
        \caption{ATE (m) on Grid (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0217_ldmk_percent_rerun_nLm.png}
        \caption{Estimated number of landmarks (relative to GT) on Grid (2D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220228_2350_odom_noise_lv_refGN.png}
        % \caption{Grid (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220228_2350_odom_noise_lv_nLm.png}
        % \caption{Grid (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0020_ldmk_t_std_refGN.png}
        % \caption{Intel (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0020_ldmk_t_std_nLm.png}
        % \caption{Parking Garage (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0050_ldmk_percent_refGN.png}
        \caption{ATE (m) on Grid (3D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0050_ldmk_percent_nLm.png}
        \caption{Estimated number of landmarks (relative to GT) on Grid (3D)}
    \end{subfigure}%
    \caption{Absolute trajectory error (ATE) with respect to the pseudo-ground-truth from running Gauss-Newton and estimated number of landmarks (relative to the ground-truth number) on the two grid datasets.}
    \label{fig:gridresults}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intelgarageresults/20220301_0454_ldmk_t_std_refGN.png}
        % \caption{Intel (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intelgarageresults/20220301_0454_ldmk_t_std_nLm.png}
        % \caption{Parking Garage (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intelgarageresults/20220301_0730_ldmk_percent_refGN.png}
        \caption{ATE (m) on Intel (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intelgarageresults/20220301_0730_ldmk_percent_nLm.png}
        \caption{Estimated number of landmarks (relative to GT) on Intel (2D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0020_ldmk_t_std_refGN.png}
        % \caption{Intel (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0020_ldmk_t_std_nLm.png}
        % \caption{Parking Garage (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0050_ldmk_percent_refGN.png}
        \caption{ATE (m) on Garage (3D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0050_ldmk_percent_nLm.png}
        \caption{Estimated number of landmarks (relative to GT) on Garage (3D)}
    \end{subfigure}%
    \caption{Absolute trajectory error (ATE) with respect to the pseudo-ground-truth from running Gauss-Newton and estimated number of landmarks (relative to the ground-truth number) on the two semi-synthetic datasets.}
    \label{fig:semisynresults}
\end{figure}

\begin{table}[tb]
    \small
    \centering
    \noindent
    \caption{
        ATE (first two rows) and run-time (sec) (last two rows) results on the two real datasets. Estimates of the number of landmarks are given in parentheses (relative to the ground-truth). To obtain the results on the corridor dataset, Alternation and K-SLAM employed a higher noise model increased from 0.1 default standard deviation to 5.5. GNC's maximum distance threshold was set to 3. For the Indoor dataset, measurement noise standard deviation was set to 0.1 throughout.
    }
    \begin{tabular}{c | c c c c c}
        \hline
        Dataset & Odom & ML & Alt & GNC & K-SLAM  \\
        \hline
        Indoor & 0.415 (+24)  & 0.833 & 0.076 & 0.157 & \textbf{0.046} (+1) \\
        Corridor & 6.67 (+233) & 7.13 & 4.18 & 5.817 & \textbf{1.068} (-233) \\
        \hline
        Indoor & n/a & 7.49 & 1.66 & 2.94 & 16.73 \\
        Corridor & n/a & 77.05 & 24.83 & 21.93 & 69.2 \\
        \hline
    \end{tabular}
    \label{tab:realresults}
\end{table}

\begin{figure}
    \centering
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/realresults/matlab_altkmfree_results.png}
        \caption{Indoor}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/realresults/kevin3000_altkmfree_results(originalGT).png}
        \caption{Corridor}
    \end{subfigure}%
    \caption{Results of running K-SLAM on the two real datasets. Black denotes the estimated trajectories and landmarks. Blue denotes the pseudo-ground-truth obtained by Gauss-Newton.}
    \label{fig:realkslam}
\end{figure}

\subsection{Results: Runtime}
\label{sec:runtime}

We analyze the run-time performance of the methods on the 2D grid dataset as shown in Fig.~\ref{fig:runtime} and the real datasets in Tab.~\ref{tab:realresults}. K-SLAM, although being accurate, is the slowest algorithm, while GNC is one of the fastest. In general, the run-time of GNC varies between the maximum likelihood method and somewhat below the alternation approach in our experiments. The run-time of all the algorithms increases linearly on the log-scale plot (Fig.~\ref{fig:runtime}) as the number of landmarks increases, indicating the combinatorial nature of the problem.

\begin{figure}
    \centering
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/runtimegrid/20220301_0217_ldmk_percent_rerun_time.png}
        % \caption{Indoor}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/runtimegrid/20220301_0257_ldmk_t_std_rerun_time.png}
        % \caption{Corridor}
    \end{subfigure}%
    \caption{Run-time on the 2D grid datasets.}
    \label{fig:runtime}
\end{figure}

==> sections/fig-gridResults.tex <==
%!TEX root = ../root.tex

\begin{figure}
    \centering
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0133_odom_noise_lv_rerun_refGN.png}
        % \caption{Grid (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0133_odom_noise_lv_rerun_nLm.png}
        % \caption{Grid (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0257_ldmk_t_std_rerun_refGN.png}
        % \caption{Intel (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0257_ldmk_t_std_rerun_nLm.png}
        % \caption{Parking Garage (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0217_ldmk_percent_rerun_refGN.png}
        \caption{ATE (m) on Grid (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0217_ldmk_percent_rerun_nLm.png}
        \caption{Estimated number of landmarks (relative to GT) on Grid (2D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220228_2350_odom_noise_lv_refGN.png}
        % \caption{Grid (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220228_2350_odom_noise_lv_nLm.png}
        % \caption{Grid (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0020_ldmk_t_std_refGN.png}
        % \caption{Intel (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0020_ldmk_t_std_nLm.png}
        % \caption{Parking Garage (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0050_ldmk_percent_refGN.png}
        \caption{ATE (m) on Grid (3D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0050_ldmk_percent_nLm.png}
        \caption{Estimated number of landmarks (relative to GT) on Grid (3D)}
    \end{subfigure}%
    \caption{Absolute trajectory error (ATE) with respect to the pseudo-ground-truth from running Gauss-Newton and estimated number of landmarks (relative to the ground-truth number) on the two grid datasets.}
    \label{fig:gridresults}
\end{figure}

==> sections/fig-nrLmks.tex <==
%!TEX root = ../root.tex

\begin{figure}
    \centering
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{figures_202209/eval_results/2dgrid/20220825_0325_odom_noise_lv_nLm_up.png}
        % \caption{Indoor}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{figures_202209/eval_results/2dgrid/20220825_0805_ldmk_t_std_nLm_up.png}
        % \caption{Corridor}
    \end{subfigure}%
    \caption{Difference between the estimated and the ground truth number of landmarks for \nameKmeans and the \nameML baseline on the 2D grid dataset with different noise levels.\label{fig:nrLmks}}
    % \vspace{-4mm}
\end{figure}

==> sections/fig-qualitativeResultsKSLAM.tex <==
%!TEX root = ../root.tex

\begin{figure}
    \centering
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/realresults/matlab_altkmfree_results.png}
        \caption{Indoor}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/realresults/kevin3000_altkmfree_results(originalGT).png}
        \caption{Corridor}
    \end{subfigure}%
    \caption{Results of running \nameKmeans on the two real datasets. Black denotes the estimated trajectories and landmarks. Blue denotes the pseudo-ground-truth obtained by Gauss-Newton.}
    \label{fig:realkslam}
\end{figure}

==> sections/fig-runtime.tex <==
%!TEX root = ../root.tex

\begin{figure}
    \centering
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{figures/runtimegrid/2d/20220301_0217_ldmk_percent_rerun_time.png}
        % \caption{Indoor}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=1.1\linewidth]{figures/runtimegrid/2d/20220301_0257_ldmk_t_std_rerun_time.png}
        % \caption{Corridor}
    \end{subfigure}%
    \caption{Runtime on the 2D grid dataset.\label{fig:runtime} \vspace{-4mm}}
\end{figure}

==> sections/fig-semisynt.tex <==
%!TEX root = ../root.tex

\begin{figure}
    \centering
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intelgarageresults/20220301_0454_ldmk_t_std_refGN.png}
        % \caption{Intel (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intelgarageresults/20220301_0454_ldmk_t_std_nLm.png}
        % \caption{Parking Garage (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intelgarageresults/20220301_0730_ldmk_percent_refGN.png}
        \caption{ATE (m) on Intel (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/intelgarageresults/20220301_0730_ldmk_percent_nLm.png}
        \caption{Estimated number of landmarks (relative to GT) on Intel (2D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0020_ldmk_t_std_refGN.png}
        % \caption{Intel (2D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0020_ldmk_t_std_nLm.png}
        % \caption{Parking Garage (3D)}
    \end{subfigure}%
    \newline
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0050_ldmk_percent_refGN.png}
        \caption{ATE (m) on Garage (3D)}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gridresults/20220301_0050_ldmk_percent_nLm.png}
        \caption{Estimated number of landmarks (relative to GT) on Garage (3D)}
    \end{subfigure}%
    \caption{Absolute trajectory error (ATE) with respect to the pseudo-ground-truth from running Gauss-Newton and estimated number of landmarks (relative to the ground-truth number) on the two semi-synthetic datasets.}
    \label{fig:semisynresults}
\end{figure}
